Sigma: Differential Rescaling of Query, Key and Value for Efficient Language Models

We introduce Sigma, an efficient large language model specialized for the system domain, empowered by a novel architecture including DiffQKV attention, and pre-trained on our meticulously collected system domain data. DiffQKV attention significantly enhances the inference efficiency of Sigma by optimizing the Query (Q), Key (K), and Value (V) components in the attention mechanism differentially, based on their varying impacts on the model performance and efficiency indicators. Specifically, we (1) conduct extensive experiments that demonstrate the model's varying sensitivity to the compression of K and V components, leading to the development of differentially compressed KV, and (2) propose augmented Q to expand the Q head dimension, which enhances the model's representation capacity with minimal impacts on the inference speed. Rigorous theoretical and empirical analyses reveal that DiffQKV attention significantly enhances efficiency, achieving up to a 33.36% improvement in inference speed over the conventional grouped-query attention (GQA) in long-context scenarios. We pre-train Sigma on 6T tokens from various sources, including 19.5B system domain data that we carefully collect and 1T tokens of synthesized and rewritten data. In general domains, Sigma achieves comparable performance to other state-of-arts models. In the system domain, we introduce the first comprehensive benchmark AIMicius, where Sigma demonstrates remarkable performance across all tasks, significantly outperforming GPT-4 with an absolute improvement up to 52.5%.

==> Sections/4_sigma_general.tex <==
\section{\textsc{Sigma}}


\subsection{Pre-training Data}
% 对于general数据，我们将DCLM以及FineWeb-EDU混合后去重，作为General Dataset Ⅰ，token数量大约为4T，经过进一步的质量过滤，我们将过滤后的数据作为General Dataset Ⅱ，数据量约为1T token。最终我们将得分更高的数据选出作为General Dataset Ⅲ，大约200B的general语料用于参与到\textsc{Sigma}的退火阶段。
% 对于math domain的数据，我们使用proof-pile-2，混合上我们从General Dataset Ⅰ中过滤的math相关的280B语料，作为数学domain的预训练数据。关于code domain的数据，我们参考Codestarv2的过滤方法，筛选了500B的code domain相关的数据集。
% 同时，我们有大约有1T左右的经过质量筛选的合成，重写的预训练语料，包含多个domain的内容，参与到预训练的后期阶段当中。
The training of \textsc{Sigma} is carried out on large-scale general data and some proprietary domain data.
For \textbf{general domain} data, we combine DCLM~\citep{li2024datacomp} and FineWeb-EDU~\citep{penedo2024fineweb} and then remove duplicates to obtain General Dataset $\mathrm{I}$. The number of tokens is approximately 4 trillion. After further quality filtering, we take the filtered data as General Dataset $\mathrm{II}$, with the number of tokens 1 trillion tokens. Finally, we select the data with higher scores and stricter rules as General Dataset $\mathrm{III}$, which contains approximately 200 billion tokens that participate in the annealing phase of \textsc{Sigma}'s pre-training.
For data in the \textbf{math domain}, we use proof-pile-2~\citep{azerbayev2023llemma} and combine it with 280 billion math-related corpora filtered from General Dataset $\mathrm{I}$ as the pre-training data for the math domain.
Regarding data in the \textbf{code domain}, we refer to the filtering method of StarcoderV2~\citep{li2023starcoder} and select the dataset related to the code domain of 500 billion tokens.
Moreover, we have approximately 1 trillion of synthesized and rewritten pre-training corpora that have undergone quality screening and contain content from multiple domains, which participate in the later phase of \textsc{Sigma} pre-training.



% 我们分别在512张A100-40G上以及256张H100上训练\textsc{Sigma}-1.5B和\textsc{Sigma}-10B。第一阶段我们用General Dataset $\mathrm{I}$混合数学domain和code domain的数据，按照General:Math:Code=8:1:1的比例进行训练，学习率峰值为1.5e-4，batch size从4M逐步扩大到16M，总训练量为4T。第二阶段我们提高了math和code的比例，并使用了进一步质量过滤后的General Dataset $\mathrm{II}$,按照General:Math:Code=4:3:3的混合比例进行训练，总训练量为1.5T。在第三阶段，我们按照6：4的比例混合了合成重写的预训练语料以及General Dataset $\mathrm{II}$进行训练，学习率drop到第一阶段峰值的20%,即3.0e-5，总训练量为1T。在最后的退火阶段，我们使用了分数最高的General Dataset $\mathrm{III}$和严格挑选的合成重写的预训练语料进行退火，学习率drop到0，总训练量为0.6T。
\subsection{pre-training Settings}
We conducted pre-training for \textsc{Sigma}-1.5B utilizing a cluster of 512 A100-40G GPUs and for \textsc{Sigma}-10B using 256 H100-80G GPUs. Initially, we combined datasets from general, mathematical, and coding domains with General Dataset I, adhering to a distribution ratio of General:Math:Code = 8:1:1. The training was carried out with a maximum learning rate of 1.5e-4, starting from a batch size of 4 million tokens, which was incrementally scaled up to 16 million tokens, culminating in a total training volume of 4 trillion tokens.

In the subsequent phase, we adjusted the data mix to favor mathematical and coding content, employing the quality-filtered General Dataset II. The mixing ratio for this phase was set to General: Math: Code = 4:3:3, with a total training volume of 1.5 trillion tokens.

For the third phase, we introduced a blend of synthesized and rewritten pre-training corpora alongside the General Dataset II at a ratio of 6: 4. This phase encompassed a total training volume of 1 trillion tokens, during which the learning rate was reduced to 20\% of its peak value, i.e., 3e-5.

Finally, in the annealing phase, we utilized General Dataset III, which was selected for its highest quality, along with meticulously chosen synthesized and rewritten pre-training corpora. The learning rate was gradually decreased to zero, concluding with a total training volume of 0.6 trillion tokens.

% \section{Sigma-General: Backbone Knowledge}

\subsection{General Domain Performance}
\label{sec:sigma-general}
\paragraph{Evaluation Setup.}
Following ~\citet{zhang2024tinyllama, chen2024dha}, we conduct a comprehensive evaluation of \textsc{Sigma} in terms of commonsense reasoning tasks, reading comprehension tasks, text understanding tasks, language proficiency, general knowledge, coding, and math problem-solving. With reference to the evaluation procedure of lm-evaluation-harness~\citep{eval-harness} and EvalPlus~\citep{evalplus}, we present the results of HellaSwag (Hella.)~\citep{zellers2019hellaswag}, OpenBookQA (ObQA)~\citep{OpenBookQA2018}, WinoGrande (Wino.)~\citep{sakaguchi2021winogrande}, ARC easy/Challenge (ARC.e/c)~\citep{clark2018think}, PIQA~\citep{bisk2020piqa}, SciQ~\citep{welbl2017crowdsourcing}, BoolQ (Bool.)~\citep{clark2019boolq}, and LogiQA (Logi.)~\citep{liu2020logiqa}. The above benchmarks evaluate the model's commonsense reasoning and text-understanding ability. We also evaluate on three general problem-solving benchmarks MMLU (5-shot)~\citep{hendrycks2020measuring}, MMLU-Pro (5-shot)~\citep{wang2024mmlu}, and BBH (3-shot)~\citep{suzgun2022challenging}, two code generation benchmarks HumanEval (0-shot)~\citep{chen2021evaluating} and  MBPP~\citep{austin2021program}, and two math problem datasets MATH (5-shot)~\citep{hendrycksmath2021} and GSM8K (5-shot)~\citep{cobbe2021training}.

\paragraph{Baselines.}
We compare the performance of \textsc{Sigma}-1.5B with the following state-of-the-art decoder-only LMs that have comparable sizes, including: TinyLlama-1.1B~\citep{zhang2024tinyllama}, Pythia-(1.0B, 1.4B)~\citep{biderman2023pythia}, OPT-1.3B~\citep{zhang2022opt}, Bloom-1.1B~\citep{muennighoff2022crosslingual}, Cerebras-GPT-1.1B~\citep{dey2023cerebras}, Phi1-1.3B~\citep{gunasekar2023textbooks}, Phi1.5-1.3B~\citep{li2023textbooks}, StableLM-2-1.6B~\citep{bellagente2024stable}, Qwen2.5-1.5B~\citep{qwen2.5}, SmolLM-1.7B~\citep{allal2024SmolLM}, DCLM-1.4B~\citep{li2024datacomp}, OLMo-1.2B~\citep{groeneveld2024olmo}, and Gemma-2B~\citep{team2024gemma}.

\input{Tables/main_result}
\input{Tables/problem_solving}
\paragraph{Commonsense Reasoning Tasks.}
The evaluation results on commonsense reasoning benchmarks are shown in \cref{tab:main_result}. All results are obtained via zero-shot prompting. According to the results, \textsc{Sigma}-1.5B achieves an outstanding average performance of 61.61 on 9 benchmarks, significantly outperforming strong baseline models such as OLMo-1.2B and OPT-1.3B on various reasoning and comprehension tasks. It also achieves comparable performance to state-of-the-art large language models such as Qwen2.5-1.5B, Gemma-2b, and DCLM-1.4B. Specifically, \textsc{Sigma} achieves top-2 performance at WinoGrande, PIQA, and SciQ, showing its broad and accurate grasp of both intuitive and logical commonsense during its pre-training on large-scale text sequences, which provides reliable knowledge backups for reasonable text completions and further task-specific tuning. Although it excels at common sense reasoning, \textsc{Sigma} shows limited performance on BoolQ and LogiQA, reflecting a moderate level of reading comprehension on option-form questions. We observe a significant decrease on these benchmarks during the annealing stage when math problem-solving ability improves, showing a potential conflict between natural and formal language understanding for small-scale models.


\paragraph{Problem-Solving Tasks.}
The evaluation results on various general problem-solving / coding / math benchmarks are shown in \cref{tab:ps_result}. According to the results, \textsc{Sigma}-1.5B achieves an average of 27.10 on all tasks, which is comparable to strong baseline models such as Phi1.5-1.3B and Gemma-2B. Specifically, our model reaches top-3 performances on all three general benchmarks: MMLU, MMLU-Pro, and BBH, showing its capability to apply world knowledge to various problem-solving scenarios. In the code domain, \textsc{Sigma} achieves 21.3\% and 30.7\% pass rates on the HumanEval and MBPP benchmarks, outperforming Phi1 on MBPP, a model customized for code generation. In the math domain, \textsc{Sigma} reaches 12.7\% and 27.75\% precision on the MATH and GSM8K benchmarks, surpassing competitive baseline models such as Phi1.5 and Gemma by a large margin. Notably, \textsc{Sigma}-1.5B maintains similar commonsense reasoning and general problem-solving capabilities to DCLM-1.4B, but greatly advances on all coding and math benchmarks. With a significant overlap between \textsc{Sigma} and DCLM's training corpus, the above results further showcase the importance of mixing math and code data within the general corpus during the early pre-training stage, which provides balanced improvement for text and program understanding and generation abilities. Though achieving competitive problem-solving skills, \textsc{Sigma} still struggles to compare with Qwen2.5 model on most problem-solving benchmarks. This gap shows that the scale and quality of pre-training data remain the key bottleneck for the performances of small-scale LLMs. Training on 18T tokens of high-quality data, Qwen2.5 gains significantly more knowledge and has greatly improved capabilities in coding and mathematics~\citep{qwen2.5}.

==> Sections/bk_method.tex <==
\section{Method}

In this section, we will demonstrate how \textsc{SIGMA} is designed and pretrained so as to enhance the efficiency of the model's inference process while ensuring its performance. We describe the details of the different rescaling strategies for Query(Q), Key(K) and Value(V) in \autoref{sec:method:rescalingQKV} as the main framework of our \textsc{SIGMA}, and illustrate how we pretrain \textsc{SIGMA} from scratch in \autoref{sec:method:pretraining}.

\subsection{Rescaling for Query, Key and Value}
\label{sec:method:rescalingQKV}
We present a model named \textsc{SIGMA}, which is composed of a more efficient transformer architecture for computing self-attention, to meet the demands of large language models in actual deployment scenarios. In practical situations, the bottleneck we often encounter is not the GPU memory consumption occupied by the model itself, but the GPU memory consumption on storing key and value(KV) brought by numerous user inputs, as well as the time consumption of accessing K and V from GPU to kernel for computation. For already deployed transformer-based models, we discuss how to minimize the GPU memory consumption caused by storing KV under limited deployment resources and we transfer the memory bound caused by variable length KV to fixed length Q to reduce the time overhead of accessing KV and maintain the performance of the model.

\paragraph{Differentially Compressed KV}
\paragraph{Augmented Q}
\paragraph{Selective V Cache Fetching}


\subsection{Pretraining of SIGMA}
\label{sec:method:pretraining}

==> Sections/bk_observations.tex <==
\subsection{Observations}
\label{sec:obs}
% 作为SIGMA模型设计的依据，我们分别对Q,K,V进行了变换以探究其对模型性能的影响。我们使用相同的100B规模的来自fineweb的语料，在1B左右的Transformer based的模型上从头预训练，在3.1中有了压缩K，V对于模型性能影响的发现，以及3.2中增强Q对于模型性能影响的发现。
In this section, we present our experimental findings on how various configurations of the Q, K, and V components in the DiffQKV attention would influence the model performance. 
To achieve this, we explore different model architectures and train them from scratch to assess their performance, entailing a substantial number of pre-training experiments.
In the following experiments, we adopt 100 billion tokens from FineWeb-Edu \citep{penedo2024fineweb} as the pre-training data. All model architectures are scaled to approximately 1 billion parameters, which consists of 22-layer transformer blocks with a hidden dimension of 2048.
%\red{(specific model hyper-parameters, such as the layer number, hidden dimension, FFN size, etc.)}.
%As the basis for the design of the \textsc{SIGMA}, we transformed Q, K, and V respectively to explore their impacts on model performance. 
%\blue{We used the same 100B corpus from FineWeb-Edu dataset \citep{penedo2024fineweb} and conducted pre-training from scratch on a Transformer-based model of around 1B in size.} 
% \cref{sec:observation:comparing_kv_compression} discusses the impacts of differentially compressing K and V components and \cref{sec:observation:augmenting_q} explores the effects of augmenting the Q component.

% \subsection{Comparing K and V Compression}
% \label{sec:observation:comparing_kv_compression}
\paragraph{Observation 1} \emph{The model performance is more sensitive to the decrease in the number of V heads ($n^h_v$) than in the number of K heads ($n^h_k$).} 
Specifically, we reduce the number of heads of K and V in the DiffQKV attention, respectively, and assess their impacts on model performance by comparing with the baseline that has the same number of KV heads. 
Based on the results shown in \cref{tab:kv_head_compression}, in most cases, reducing the number of K heads has a relatively minor impact on model performance compared to reducing the number of V heads. 
This differential impact is reasonable, considering the distinct roles played by the K and V components within the attention mechanisms. 
The K heads primarily serve to compute attention matrices, which prove to have a remarkable sparsity exceeding 95\% during inference \citep{zhang2024h2o}. This high sparsity nature implies that a slight decrease in the parameters used for its calculation can still yield a precise approximation. 
In contrast, the V vectors, which directly influence the final attention output, demands a more nuanced approach.
% In contrast, as V is the value obtained by weighting to get the final attention output, more calculations on it maybe more worthwhile.
% 具体来说，我们分别降低K和V的head的数量，将其和具有相同KV head的数量的baseline进行比对，以探究其对模型性能带来的影响。从表1的结果来看，当head个数分别为32，16，8，4，1的时候，降低k的head数量相比于降低v的head的数量对模型性能的影响是更小的。
% We believe that although K participates in the calculation of attention score, a slight loss of attention score may have little impact on the final attention output. 
\input{Tables/kvhead_exp}
% 我们认为k虽然参与attention score的计算，但是attention score的轻微损失可能对最终的计算结果影响较小，而v作为加权得到最终输出的value，更多在它上面的计算是值得的。
% or we need more exp?

\input{Tables/minik_dim_exp}
\paragraph{Observation 2} \emph{Reducing the dimension of K heads to half of the dimension of V heads ($d^h_k = d^h_v/2$) can preserve the model performance, compared to the scenario where the dimensions of K and V heads are equal ($d^h_k = d^h_v$).} %工作表4
% 一般来说，减少K的维度和减少K的head的数量是从两个不同的维度上对K进行压缩。为了与head维度压缩的K对应以计算attention score，我们需要将Q的head维度映射到和K的head维度相同，这可能会带来一定程度上的损失。因此我们保持K和V的head数量相同，并减少K的head维度，以观察压缩K的head维度对模型性能带来的影响。从表2的结果可以看到，在大部分情况下，压缩K的head维度对模型整体性能带来的损失是比较小的，甚至部分head数量设置的情况下，更小的K的维度能带来与压缩前相当的性能。
In Observation 1, we showcase the minial effects resulting from a decrease in the number of K heads. Here, we explore an alternative approach to compressing K components by reducing the dimension of K heads. More specifically, ``the dimension of K heads'' refers to $d^h_k$ in \cref{sec:diffQKV} and its reduction indicates a smaller $W_K$ and $k_t$). To compute the attention scores when the dimensions of K and V are different (\cref{eq:diffqkv_att_score}), we transform the dimension of $K$ to the same as $V$ through a trainable feedforward layer.
In essence, this operation of reducing K head dimension helps conserve the memory usage caused by KV cache at the cost of additional computation from a feedforward layer. This tradeoff can be very cost-effective as the primary bottleneck for LLM inference speed lies in memory bandwidth rather than computation \citep{shazeer2019fast, ribar2024sparq}. 
%Generally, reducing the dimension of K and reducing the number of heads of K are two different aspects to compress K. 
%In order to calculate the attention score corresponding to K compressed in the head dimension, we need to map the head dimension of Q to be the same as that of K, which may bring a certain degree of model performance. Therefore, we keep the same number of KV heads and reduce the head dimension of K to observe the impact of compressing the head dimension of K on the model performance. 
To investigate the impact of reducing K head dimension, we conduct a comparison of various attention settings, such as MHA and GQA, along with their counterparts having only half of the K head dimension. 
The results presented in \cref{tab:k_headdim_compression} demonstrate that the decrease in performance due to reducing the K head dimension is negligible. In certain configurations, the model with a smaller K head dimension even outperforms the baseline setting prior to compression. 
%As shown by results in \autoref{tab:k_headdim_compression}, the performance loss caused by compressing the head dimension of K is minimal. In some settings of the number of heads, the model with smaller K head dimension even achieves slightly superior performance compared with the baseline setting before compression. 

% topK value
% 通过attention score选出score最高的那部分V参与到最后attention out计算当中就可以维持模型的大部分性能
\input{Tables/topkV_exp}
\paragraph{Observation 3} \emph{Using only a small proportion of V vectors, specifically those corresponding to the highest attention scores, in the attention output calculation can still preserve the model performance.}
% \paragraph{Observation 3} \emph{Leaving the top-k V calculated through the attention score to participate in the final attention output calculation can effectively maintain most of the performance of the model.}
% 在之前我们发现压缩K的损失小于压缩V的损失，然而V会带来更多的KV cache开销。如果我们能利用计算好的attention score选择需要的value，就可以显著降低V在推理计算过程中cache的消耗。简单取前k高attention score位置的value，就可以让模型在选择少量value的情况下最大程度保持模型原先的性能。如表3结果所示，在top100 value的设置下，模型就能够保持和原先模型相当的效果，并且可以节省value的cache操作带来的开销。
As in previous work, topk V can improve the memory-efficiency of the model~\citep{gupta2021memory}, inspiring us to adopt this strategy in this KV imbalance scenario.
As shown in \cref{tab:topkV}, even when we only use 100 V vectors corresponding to the top-100 highest attention scores (denoted as ``Sel.V-top100''), the model can still maintain a comparable effect to the original setting. % (GQA, MHA) and save the overhead caused by cache operations of values.
%Previously, we found that the loss of compressing K is smaller than that of compressing V. However, V incurs more overhead for KV cache. 
These results indicate that we only need to retrieve a small proportion of V vectors from the cache during inference to achieve competitive performance. This can significantly reduce data transfer and demand on memory bandwidth, thereby improving inference speed.
% Assume we can use the computed attention scores to select the required values, the consumption of cache for V during the inference can be significantly reduced. 
% Simply taking the values at the positions with the top k attention scores can maintain the performance of the model, so that only a small number of values participate in the final calculation.
% As shown in \autoref{tab:topkV}, under the setting of Sel.V-top100 (selct top100 value), the model can maintain a comparable effect to the original model(GQA, MHA) and save the overhead caused by cache operations of values.

% \subsection{Augmented Q} % Head Dimension}
\label{sec:observation:augmenting_q}
Augmenting the self-attention layer with extra parameters is a straightforward way to enhance its representational capacity and improve model performance. 
Since the Q vectors in self-attention do not need to be cached during inference, their impact on memory usage and data transfer duration is minimal. Therefore, investing extra parameters in the Q components can be more cost-effective compared to the KV components. In the following, we investigate whether augmenting Q components can boost model performance through experiments.

%To make up for the loss caused by compressing K and V, and considering the importance of self-attention in the entire Transformer architecture, we need to increase the parameters of attention layer at a minimal cost to enrich its characterization ability.
%Considering that the sequence length of the Q head is only 1 during inference, it is more reasonable to add additional parameters to Q to improve the model's performance in attention. 

\input{Tables/largeq_exp}
% Augmenting the dimension of Q这个描述现在似乎不太准确
% \paragraph{Observation 4} \emph{Augmenting the dimension of Q heads ($d_q^h$) can boost model performance. } %工作表5

% 为了弥补压缩k,v带来的损失，同时考虑到self-attention在整个Transformers架构中的重要性，我们需要以尽量小的代价增加attention层的参数量以丰富其表征的内容。考虑到Q head在推理的过程中序列长度仅为1，在Q上添加额外的参数来提高模型在Attention上的性能更加合理。为了进一步探究在Q上引入额外的参数是否能够给模型的性能带来进一步的提升，我们在Q上引入不同规模的参数量来探究其对于模型性能的影响。从表3的结果可以看到，在Q上引入额外的参数量可以使得模型的性能有不同程度上的提升，尤其在KV压缩程度较高的时候提升更为明显。($n^h_v$=4,$n^h_k$=4)从最终模型性能表现上来看，1.5×(q\_intermediate\_size\=3072)的放缩更为合适。
\paragraph{Observation 4} \emph{Augmenting Q components can boost model performance. } %工作表5
%We investigate whether introducing additional parameters on Q can bring improvement to the model's performance. 
In our experiments, we varied the number of parameters in Q to assess their impact on model performance. As demonstrated in \cref{tab:large_q}, adding extra parameters to Q can enhance the model's performance to different extents, especially when the compression levels of K and V are higher ($n^h_v$=4,$n^h_k$=4).
Based on the overall model performance, a scaling factor of 1.5$\times$ (i.e. $d_q^h = 3072$) seems to be optimal.
%In our experiments, we introduce different amounts of parameters on Q to explore their impact on model performance. As results shown in \autoref{tab:large_q}, introducing additional parameters on Q can improve the model's performance to varying degrees, especially when the compression degree of K and V is higher ($n^h_v$=4,$n^h_k$=4). Judging from the final model performance, a scaling factor of $1.5\times$ (q\_intermediate\_size = 3072) is more appropriate.


% \paragraph{Observation 5} \emph{With an equal amount of extra parameters, the performance gain from augmented Q is superior to that from expanding the FFN module. } %工作表10

% 
\input{Tables/largeq_mlp_exp}
\paragraph{Observation 5} \emph{With an equal number of addtional parameters, the performance gain from augmenting Q is superior to that from expanding the FFN module. Furthermore, the performance gains from augmenting Q and expanding the FFN module are independent of each other. In other words, with a fixed augmented Q, further enlarging the FFN module continues to enhance model performance. }
% 具体地，我们讨论基于标准Transformer，分别在FFN和Q上增加同样规模的参数量，研究其对于模型表现的影响。在表5的实验设置中，隐藏层维度和增加的参数量成正比例关系，可以发现在Q上增加参数量的模型性能始终由于在FFN上增加参数模型的性能，这一点尤其在FFN的隐藏层维度较大的时候更为明显，例如，在FFN上增加的参数量是Q的两倍（3072*2），但是模型性能还是略逊于后者。这侧面反映了在FFN上增加参数量对模型的提升是存在瓶颈的，而在Q上增加参数从Transformer块参数量分布上来看是一个更加高效的选择。
By adding the same number of parameters to the FFN and Q modules, respectively, we examine and compare their impacts on the model performance. %According to the experimental setting in \autoref{tab:large_q_vs_mlp}, the hidden layer dimension is in a proportional relationship with the amount of parameters. 
According to the results shown in \cref{tab:large_q_vs_mlp}, the performance enhancement yielded by augmented Q is consistently more obvious than adding the same number of parameters in the FFN module. %it can be found that the model performance with parameters on Q is always better than on FFN, which is more obvious when the hidden layer dimension of FFN is larger. 
By comparing the last two lines of results in \cref{tab:large_q_vs_mlp}, we can observe that even when the number of additional parameters on FFN (2$\delta$) is twice that of Q ($d^h_q=\delta$), the model performance is still slightly inferior to the latter. 
These results indicate that adding parameters on the self-attention layer can more effectively improve model performance than on the FFN module.
%This indirectly reflects that there is a bottleneck in improving the model by increasing the amount of parameters on FFN, and increasing parameters on Q is a more efficient choice in terms of the parameter distribution of the Transformer block. 



%总体来说，相对于压缩V，压缩K给模型性能带来的损失是更小的，并且从K的head数量和K的维度对K进行压缩都看起来是可以接受的做法。同时，为了确保没有压缩的V在Attention计算过程中开销尽量小，根据topK的attention分数来选择V是一个高效的选择。另外，为了确保最终self-attention计算的质量，我们在Q上引入额外ca
\input{Tables/combine_exp}
\subsection{Summary: Optimal Configuration for DiffQKV Attention}
\label{sec:obs_sum}
Based on the above observations, we can summarize the optimal configurations for DiffQKV attention that can well balance model performance and inference efficiency as follows: 1) \emph{differentially compressed KV}: Unlike compressing V components, compressing K incurs less performance degradation, whether in terms of the number of K heads~($n^h_k$) or the dimension of K~($d^h_k$); %Furthermore, compressing K, whether in terms of the number of K heads~($n^h_k$) or the dimension of K~($d^h_k$), appears to be an admissible methodology. 
2) \emph{selective V cache fetching}: the efficiency for loading the non-compressed V components can be optimized by only selecting a small proportion of 
V vectors, corresponding to the highest attention scores, to approximate the calculation; %for participation in the final computation based on the top k attention scores, thereby augmenting the efficiency of the actual attention computation. 
3) \emph{augmented Q}: introducing extra parameters to the Q components can enhance the representational capacity of the self-attention layer, while having a relatively small impact on inference efficiency, since the Q vectors do not need to be cached during inference. %, we can introduce extra parameters to Q to alleviate the bottleneck of the model within the attention mechanism, thus diminishing the performance loss of the model. 
In \cref{tab:combine_exp}, by integrating three aforementioned strategies (i.e., -75\% K Heads ($n_k^h$=4), Half K Dim($d^h_k = d^h_v/2$), and AugQ ($d_q^h$=3072), we observe that the model's performance surpasses that of the original model and also exhibits advantages in terms of inference speed and KV cache utilization.

In summary, by employing an imbalanced KV head, we have developed a more efficient model architecture. Furthermore, the introduction of the augmented Q module allows us to compensate for the loss incurred by compression while achieving superior performance compared to standard models. The implications of this approach extend beyond the \textsc{Sigma} model, particularly in light of recent trends toward increasing model capacity. To conserve the KV cache overhead during inference in large models, there has been a gradual trend towards reducing the proportion of attention mechanism parameters within the entire Transformer block. Given the critical role of the attention mechanism in language models, its compression cannot be done without limits. By reinforcing the Q head that does not require caching, our method introduces new possibilities for scaling up the attention mechanism, thereby enriching its representational space. \cref{tab:large_q_vs_mlp} highlights the parameter efficiency gained from scaling up the parameters of the attention mechanism.
However, incorporating the augmented Q inevitably introduces additional inference costs. We will further elucidate the practical efficiency of \textsc{Sigma} in \cref{sec:efficiency_analysys}.



\subsection{Model Architecture}
\label{sec:architecture}
Building on the insights of the DiffQKV attention discussed in \cref{sec:obs_sum}, we construct \textsc{Sigma}, a pre-trained language model characterized by strong performance and inference efficiency. 
% In this section, we illustrate the specific architecture adopted by \textsc{Sigma}, its training procedure and its performance in the general domain. The efficiency analysis of \textsc{Sigma} is provided in \S\ref{sec:efficiency_analysys}. 
% \textsc{Sigma} 的训练在大规模的General数据上以及一些专有Domain的数据上进行。我们使用全新的模型架构，并在general的benchmark上以及ads和system domain上测试了我们模型的性能。我们将在下面介绍详细的内容。
%The training of \textsc{Sigma} is carried out on large-scale general data and some proprietary domain data. We use a brand new model architecture and have tested the performance of our model on general benchmarks as well as \red{industry benchmarks on the ADS and SYSTEM}. We will introduce the detailed content below.
% 在\textsc{Sigma}的训练上，我们分别使用了两种不同参数量规模的模型，分别有1.5B的参数和10B的参数。为了兼顾模型表现和KV cache的开销，我们在训练\textsc{Sigma}1.5B和\textsc{Sigma}10B时并没有对k的维度进行压缩，仅减少了K head的数量。具体来说，我们设置K head=4，v的head个数为Q的head个数的一半，设置为V head=16。在\textsc{Sigma}-1.5B上，我们设置$d_q^h$=3072，\textsc{Sigma}-10B上设置为$d_q^h$=6144，对应于1.5倍的hidden state维度，以扩展Q的表征空间。我们使用和Llama3一样的词表，词表大小为128k。
%Regarding the selection of \textsc{Sigma} architectures, 
Specifically, we adopt two model scales with 1.5 billion parameters and 10 billion parameters, respectively (i.e. \textsc{Sigma}-1.5B and \textsc{Sigma}-10B). 
For the sake of balancing the model performance and the cost of the KV cache, during the training of \textsc{Sigma}-1.5B and \textsc{Sigma}-10B, no dimension compression is applied to the K heads. Only the number of K heads was decreased. Concretely, the K head is set to 4, and the number of V heads, which is half of the number of Q heads, is set to 16.
For \textsc{Sigma}-1.5B, we set $d_q^h=3072$, and for \textsc{Sigma}-10B, we set $d_q^h=6144$, corresponding to 1.5 times the dimension of the hidden state, so as to extend the representational space of Q.
We utilize the same vocabulary as Llama3 \citep{dubey2024llama}, with a vocabulary size of 128k.
For more detailed configurations of the \textsc{Sigma} architecture, please refer to \cref{tab:hyperparameters}.

\input{Tables/hyperparameters}

==> Sections/bk_sigma2b_general.tex <==
% \section{Experimental Results}
% \subsection{Experimental Setup}
% We used two models with different parameter scale sizes, with 1.5 billion parameters and 10 billion parameters respectively(i.n. \textsc{Sigma}-1.5B, \textsc{Sigma}-10B). We set $n_k^h = 4$, $n_v^h = 16$, and set the Q intermediate size of the 1.5B model to 3072, and that of the 10B model to 6144, corresponding to 1.5 times the hidden state dimension (i.e., 2048 and 4096). To balance the trade-offs in performance, we did not compress the dimension of k when training \textsc{Sigma}-1.5B and \textsc{Sigma}-10B, and only reduced the number of its heads. We use the same vocabulary as Llama3, with the vocabulary size being 128k

% 我们遵循已有的工作（Tinyllama和DHA），在Commonsense reasoning任务，reading comprehension任务，文本理解任务，语言能力，通用知识方面上对\textsc{Sigma}进行评估。参照lm-evaluation-harness的评估流程，我们报告HellaSwag(Hella.), OpenBookQA(ObQA), WinoGrande(Wino.), ARC Challenge(ARC.), PIQA, SciQ, BoolQ(Bool.), LogiQA(Logi.), LAMBADA(LAMB.), MMLU(5-shot)的结果。
% TODO: BBH, AGIEVAL, HumanEval, DROP, MMLU-Pro, MBPP, math, gsm8k



% TinyLlama-1.1B, Pythia-1.0B, Pythia-1.4B, OPT-1.3B, Galactica-1.3B, Bloom-1.1B, Cerebras-GPT-1.1B, phi1-1.3B, phi1.5-1.3B, StableLM-2-1.6B, Qwen 2.5 1.5B, Gemma-2B, SmolLM-1.7B, DCLM-1.4B, OLMo-1.2B   


% 我们在评估\textsc{Sigma}预训练后的模型性能, 与当前常见的<2B量级的模型baseline进行对比。如表1展示的结果，在各项能力上，\textsc{Sigma}相较于现有的baseline都有极具竞争力的表现。并与当前主流开源模型phi-1.5b，llama-1b，dclm-1.4b等具有可比较的水平。

\section{Sigma-General: Backbone Knowledge}
\label{sec:sigma-general}
\subsection{General Domain Performance}
\paragraph{Evaluation Setup}
Following ~\citep{zhang2024tinyllama, chen2024dha}, we conduct comprehensive evaluation of \textsc{Sigma} in terms of commonsense reasoning tasks, reading comprehension tasks, text understanding tasks, language proficiency, general knowledge, coding, and math problem solving. With reference to the evaluation procedure of lm-evaluation-harness~\citep{eval-harness} and EvalPlus~\citep{evalplus}, we present the results of HellaSwag (Hella.)~\citep{zellers2019hellaswag}, OpenBookQA (ObQA)~\citep{OpenBookQA2018}, WinoGrande (Wino.)~\citep{sakaguchi2021winogrande}, ARC easy/Challenge (ARC.e/c)~\citep{clark2018think}, PIQA~\citep{bisk2020piqa}, SciQ~\citep{welbl2017crowdsourcing}, BoolQ (Bool.)~\citep{clark2019boolq}, and LogiQA (Logi.)~\citep{liu2020logiqa}. The above benchmarks evaluate model's commonsense reasoning and text understanding ability. We also evaluate on three general problem solving benchmarks MMLU (5-shot)~\citep{hendrycks2020measuring}, MMLU-Pro (5-shot)~\citep{wang2024mmlu}, and BBH (3-shot)~\citep{suzgun2022challenging}, two code generation benchmarks HumanEval (0-shot)~\citep{chen2021evaluating} and  MBPP~\citep{austin2021program}, and two math problem datasets MATH (5-shot)~\citep{hendrycksmath2021} and GSM8K (5-shot)~\citep{cobbe2021training}.

\paragraph{Baselines}
We compare the performance of \textsc{Sigma}-1.5B with the following state-of-the-art decoder-only LMs that have comparable sizes, including: TinyLlama-1.1B~\citep{zhang2024tinyllama}, Pythia-(1.0B, 1.4B)~\citep{biderman2023pythia}, OPT-1.3B~\citep{zhang2022opt}, Bloom-1.1B~\citep{muennighoff2022crosslingual}, Cerebras-GPT-1.1B~\citep{dey2023cerebras}, Phi1-1.3B~\citep{gunasekar2023textbooks}, Phi1.5-1.3B~\citep{li2023textbooks}, StableLM-2-1.6B~\citep{bellagente2024stable}, Qwen2.5-1.5B~\citep{qwen2.5}, SmolLM-1.7B~\citep{allal2024SmolLM}, DCLM-1.4B~\citep{li2024datacomp}, OLMo-1.2B~\citep{groeneveld2024olmo}, and Gemma-2B~\citep{team2024gemma}.

\input{Tables/main_result}
\input{Tables/problem_solving}
\paragraph{Commonsense Reasoning Tasks.}
The evluation results on commonsense reasoing benchmarks are shown in \cref{tab:main_result}. All results are obtained via zero-shot prompting. According to the results, \textsc{Sigma}-1.5B achieves an outstanding average performance of 61.61 on 9 benchmarks, significantly outperforming strong baseline models such as OLMo-1.2B and OPT-1.3B on various reasoning and comprehension tasks. It also achieves comparable performance to state-of-the-art large language models such as Qwen2.5-1.5B, Gemma-2b, and DCLM-1.4B. Specifically, \textsc{Sigma} achieves top-2 performance at WinoGrande, PIQA, and SciQ, showing its broad and accurate grasp of both intuitive and logical commonsense during its pretraining on large-scale text sequences, which provides reliable knowledge backups for reasonable text completions and further task-specific tuning. Although it excels at common sense reasoning, \textsc{Sigma} shows limited performance on BoolQ and LogiQA, reflecting a moderate level of reading comprehension on option-form questions. We observe a significant decrease on these benchmarks during the annealing stage when math problem solving ability improves, showing a potential conflict between natural and formal language understanding for small-scale models.


\paragraph{Problem Solving Tasks.}
The evluation results on various general problem solving/coding/math benchmarks are shown in \cref{tab:ps_result}. According to the results, \textsc{Sigma}-1.5B achieves an average of 27.10 on all tasks, which is comparable to strong baseline models such as Phi1.5-1.3B and Gemma-2B. Specifically, our model reaches top-3 performances on all three general benchmarks: MMLU, MMLU-Pro, and BBH, showing its capability to apply world knowledge to various problem solving scenarios. In the code domain, \textsc{Sigma} achieves 21.3\% and 30.7\% pass rates on the HumanEval and MBPP benchmarks, outperforming Phi1 on MBPP, a model customized for code generation. In the math domain, \textsc{Sigma} reaches 12.7\% and 27.75\% precision on the MATH and GSM8K benchmarks, surpassing competitive baseline models such as Phi1.5 and Gemma by a large margin. Notably, \textsc{Sigma}-1.5B maintains similar commonsense reasoning and general problem solving capabilities to DCLM-1.4B, but greatly advances on all coding and math benchmarks. With a signficant overlap between \textsc{Sigma} and DCLM's training corpus, the above results further showcase the importance of mixing math and code data within the general corpus during the early pre-training stage, which provides balanced improvement for text and program understanding and generation abilities. Though achieving competitive problem solving skills, \textsc{Sigma} still struggles to compare with Qwen2.5 model on most problem solving benchmarks. This gap shows that the scale and quality of pretraining data remain the key bottleneck for performances of small-scale LLMs. Training on 18T tokens of high-quality data, Qwen2.5 gains significantly more knowledge and has greatly improved capabilities in coding and mathematics~\citep{qwen2.5}.

==> Tables/sigma_system.tex <==
\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{5pt}
\caption{sigma\_system}
\vspace{0.5em}
\label{tab:sigma_system}
\resizebox{\linewidth}{!}{
\begin{tabular}{c cc cc cc}
\toprule
\multirow{3}{*}{\textbf{Model}} & \multicolumn{2}{c}{\textbf{Easy Reasoning}} & \multicolumn{2}{c}{\textbf{Medium Reasoning}} & \multicolumn{2}{c}{\textbf{Hard Reasoning}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}

&\textbf{Nvidia} & \textbf{AMD} & \multicolumn{2}{c}{\textbf{OptiFlow}} & \textbf{InfraWise} & \textbf{Detection} \\
& ACC & ACC & Valid Rate & Improved Rate & ACC & F1 \\
\midrule
GPT-4 & 0.2500 & 0.1700 & 0.1680 & 0.0050 & 0.1866 & 0.1670 \\
Llama3-8B-Instruct & 0.0350 & 0.0155 & 0.1640 & 0.0110 & 0.0648 & 0.0000 \\
SIGMA-System & 0.6900 & 0.6269 & 0.8670 & 0.6670 & 0.2832 & 0.1673 \\
\bottomrule
\end{tabular}
}
\end{table*}

==> Tables/sigma_system_benchmark.tex <==
\begin{table*}[h]
\centering
\small
\caption{\textsc{AIMicius} benchmark results for selected models. All metrics are normalized to a scale of 0 to 100, with higher values indicating better performance. \textbf{Bolded metrics} represent the most critical evaluation criteria for each task. \textsc{Sigma-System} 10B and \textsc{Sigma-System} (LoRA) are fine-tuned (SFT) using our proprietary dataset.}
\begin{tabular}{*{2}{l}*{4}{c}}
\toprule
% \multicolumn{6}{c}{\bf Model Performance on \textsc{AIMicius} Benchmark} \\
% \midrule
\bf Task & \bf Metric ($\uparrow$) & \bf GPT-4 & \bf \makecell{\bf Llama3-8B \\ \bf -Instruct} & \bf \makecell{\textsc{Sigma} \\ \bf \textsc{-System}} & \bf \makecell{\textsc{Sigma} \\ \bf \textsc{-System} (LoRA)} \\
\midrule
\multirow{6}{*}{\makecell[l]{\bf CMDGen \\ \bf NVIDIA}}
& CMD Score & 84.0 & 33.6 & \underline{87.5} & \bf 91.8 \\ 
& Output Score & 61.0 & 12.0 & \underline{80.9}  & \bf 85.3 \\
& Calibration Score & 62.0 & 5.0 & \underline{78.0}  & \bf 83.5 \\
& Exact Match & 13.0 & - & \bf 57.0 & \underline{52.0} \\
& Success Ratio & 21.0 & 3.5 & \underline{74.0} & \bf 77.5 \\ 
& \bf Accuracy & 25.0 & 3.5 & \underline{74.5} & \bf 77.5 \\
\midrule
\multirow{6}{*}{\makecell[l]{\bf CMDGen \\ \bf AMD}}
& CMD Score & 73.0 & 31.4 & \bf 88.9 & \underline{87.1} \\
& Output Score & 49.0 & 14.1 & \bf 78.0 & \underline{75.8} \\
& Calibration Score & 43.0 & 2.6 & \bf 79.3 & \underline{75.1} \\
& Exact Match & 14.0 & - & \bf 53.9 & \underline{48.2} \\
& Success Ratio & 13.0 & 1.6 & \bf 69.4 & \underline{66.8} \\ 
& \bf Accuracy & 17.0 & 1.6 & \bf 69.4 & \underline{67.4} \\
\midrule
\multirow{7}{*}{\bf Infrawise}
& Target & 40.7 & 28.1 & \bf 95.2 & \underline{87.5} \\
& Baseline & 34.1 & 34.5 & \bf 92.9 & \underline{88.4} \\
& Criterion & 55.1 & 11.1 & \bf 75.1 & \underline{65.6} \\
& Workload & 52.1 & 14.2 & \bf 48.4 & \underline{47.9} \\
& DCW & 22.5 & 4.6 & \bf 40.3 & \underline{34.7} \\
& Benchmark Result Recall & 19.8 & 6.5 & \bf 28.3 & \underline{25.4} \\
& \bf Benchmark Result Accuracy & 18.7 & 6.5 & \bf 28.3 & \underline{25.4} \\
\midrule
\multirow{4}{*}{\bf Optiflow}
& Code Detected & 95.8 & \underline{98.2} & \bf 100.0 & \bf 100.0 \\
& Code Executable & 50.3 & 51.2 & \underline{85.9} & \bf 97.6 \\
& \bf Plan Valid & 16.8 & 16.4 & \underline{86.7} & \bf 97.6 \\
& \bf Plan Improved & 0.5 & \underline{1.1} & \bf 66.7 & - \\
\midrule
\multirow{6}{*}{\bf NL2KQL}
& \bf Syntax Accuracy & \bf 100.0 & \underline{83.7} & \bf 100.0 & \bf 100.0 \\
& Similarity & 31.8 & 33.6 & \bf 34.9 & \underline{34.5} \\
& \bf Cluster Score & - & - & \underline{43.0} & \bf 45.4 \\
& \bf Database Score & 2.3 & 2.3 & \underline{40.7} & \bf 45.4 \\
& Table Score & 4.7 & 4.7 & \underline{17.4} & \bf 20.9 \\
& Column Score & 17.3 & 20.8 & \underline{29.0} & \bf 30.6 \\
\bottomrule
\end{tabular}
\label{tab:sigma_system_b}
\end{table*}

==> Tables/sigma_system_mtl.tex <==
\begin{wraptable}{L}{.65\linewidth}
\centering
\small
\caption{Preliminary results comparing benchmark results obtained using individual datasets versus mixed datasets. }
\begin{tabular}{*3c|*3c}
\toprule
% \multicolumn{6}{c}{\bf Prelinimary Results} \\
% \midrule
\multicolumn{3}{c|}{\bf Tasks Involved} & \multicolumn{3}{c}{\bf Task Score} \\
\midrule
\bf Task A & \bf Task B & \bf Task C & \bf Task A & \bf Task B & \bf Task C \\
\midrule
\checkmark & & & \bf 69.0 & - & - \\
& \checkmark & & - & 27.6 & - \\
& & \checkmark & - & - & \bf 41.3 \\
\midrule
\checkmark & \checkmark & & \underline{68.5} & \underline{28.7} & - \\
\checkmark & \checkmark & \checkmark & 59.0 & \bf 28.9 & \bf 41.3 \\
\bottomrule
\end{tabular}
\label{tab:sigma_system_mtl}
\end{wraptable}
